Far-Field Compression for Fast Kernel Summation Methods in High Dimensions

We consider fast kernel summations in high dimensions: given a large set of points in $d$ dimensions (with $d \gg 3$) and a pair-potential function (the {\em kernel} function), we compute a weighted sum of all pairwise kernel interactions for each point in the set. Direct summation is equivalent to a (dense) matrix-vector multiplication and scales quadratically with the number of points. Fast kernel summation algorithms reduce this cost to log-linear or linear complexity. Treecodes and Fast Multipole Methods (FMMs) deliver tremendous speedups by constructing approximate representations of interactions of points that are far from each other. In algebraic terms, these representations correspond to low-rank approximations of blocks of the overall interaction matrix. Existing approaches require an excessive number of kernel evaluations with increasing $d$ and number of points in the dataset. To address this issue, we use a randomized algebraic approach in which we first sample the rows of a block and then construct its approximate, low-rank interpolative decomposition. We examine the feasibility of this approach theoretically and experimentally. We provide a new theoretical result showing a tighter bound on the reconstruction error from uniformly sampling rows than the existing state-of-the-art. We demonstrate that our sampling approach is competitive with existing (but prohibitively expensive) methods from the literature. We also construct kernel matrices for the Laplacian, Gaussian, and polynomial kernels -- all commonly used in physics and data analysis. We explore the numerical properties of blocks of these matrices, and show that they are amenable to our approach. Depending on the data set, our randomized algorithm can successfully compute low rank approximations in high dimensions. We report results for data sets with ambient dimensions from four to 1,000.

==> lafmm_sisc_old_experiments.tex <==


We now turn to our experimental results.  We begin with an overview of our methods, then present numerical results. 
First, we show that the subblocks of a kernel matrix can be significantly compressed with an interpolative decomposition without overwhelming loss of accuracy.  Second, the decomposition can  be computed accurately by only examining a fraction of the rows of the submatrix. Finally, we present evidence that our approach works on high-dimensional data when the intrinsic dimension is low. 

\subsection{Experimental Setup}

The basic experimental setup is as follows:
\begin{enumerate}
\item Generate a set of points $D$ from some distribution $\mathcal{D}$.
\item Divide the points into three sets, sources $S$, targets $T$, and others. We specify the number of source points $m$. We take $S$ to be the set of $m$ points closest to the origin. Let $R_S$ be the distance between the origin and the farthest point in $S$.  We then let $T$ be the set of all points $y \in D$ such that $d(x, y) > D_{WS} \cdot R_S$ for a specified well-separatedness parameter $D_{WS}$, and let $|T| = N$. 
\item For a given kernel function $K(\cdot, \cdot)$, let $K$ be the $N \times m$ matrix with $K_{i,j} = K(x_i, y_j)$ for $x_i \in T$, $y_j \in S$. 
%\item Fix an approximation tolerance $\epsilon$. 
\item Choose a subsampling scheme $\mathcal{S}$ and associated parameters. Let $K_{s}$ be the subsampled approximation of $K$. 
\item Compute the numerical rank $r$ of $K_s$ with tolerance $\epsilon$ -- i.e. the number of singular values of $K_s$ greater than $\epsilon \cdot \sigma_1(K_s)$. Compute a rank $r$ decomposition of $K_s$ (either the ID or SVD).
\item Compute and report the relative error of this approximation as
\begin{equation}
E = \frac{\|\hat{K} - K\|_2}{\|K\|_2}
\label{eqn_relative_approx_error}
\end{equation}
where $\hat{K}$ is the reconstruction of the entire kernel matrix from the rank $r$ decomposition of $K_s$. 
\end{enumerate}

\textbf{Decompositions.} As noted previously, we primarily focus on the interpolative decomposition (ID). For a given matrix $A$, we compute a subset of its column indices $I$ and a matrix $P$ such that $A_I P \approx A$, where $A_I$ is the submatrix of $A$ consisting of the columns of $A$ in the index set $I$. In our subsampling experiments, we compute $I$ and $P$ from the matrix $K_s$.  We then compute the error from $K_I P$, where $K_I$ consists of the full columns of $K$ corresponding to indices in $I$. 

For comparison, we also employ the SVD, which is known to be the optimal fixed-rank approximation in terms of Frobenius and spectral norm. Our rank $k$ approximation in this case consists of the first $k$ left singular vectors in a matrix $U_k$.  We compute the approximation error by computing $U_k$ from the SVD of $K_s$.  We then compute the error caused by projecting the original matrix onto the space spanned by these vectors -- i.e. $\hat{K} = U_k U_k^T K$.

%
%
%These experiments have the following degrees of freedom:
%\begin{itemize}
%\item $\mathcal{D}$ -- the input distribution and associated parameters, especially the \emph{dimension} $d$. In particular, we are interested in distributions with a large ambient dimension, but which actually lie on a smaller dimensional (possibly nonlinear) manifold. Or, more generally, which have a small intrinsic dimension in some sense. 
%\item $m \in \mathbb{N}$ -- the size of the source set. This needs to be something large enough to allow for effective compression, but small enough so that it is a reasonable use case. For now, $m \leq 2000$ seems to be a sensible bound.  It can be as low as we can still get compression. 
%\item $D_{WS} \in [0, \infty)$ -- the well-separatedness parameter used to choose $T$. For the Laplace kernel, this can just be set to 4 in keeping with the standard notion of well-separatedness from the FMM. For other kernels, this becomes more sensitive.  In particular, for the Gaussian, it seems that the effectiveness of the compression depends on the relationship between $D_{WS}$ and the bandwidth. 
%\item $K(\cdot, \cdot)$ -- the kernel function and associated parameters, especially the \emph{bandwidth} $h$. 
%\item $\epsilon$ -- the approximation parameter used in the decomposition.  We take a number of columns $r$ such that $\sigma_{r+1}(K_s) / \sigma_1(K_s) < \epsilon$. However, this may be sensitive to the subsampling method, since we do not always know if the spectrum of the subsampled matrix corresponds to the spectrum of the full matrix.
%\item $\mathcal{S}$ -- the subsampling scheme and associated parameters, especially the \emph{sampling rate} $s$.
%\end{itemize}
%

\textbf{Subsampling Methods.} We show results for several subsampling methods, each characterized by a parameter $s$: 
\begin{itemize}
%\item \textbf{Choosing Entries} -- method of Achlioptas et al. \cite{}.  We choose an entry $K_{i,j}$ with probability $s$ (and scale it) and let it be zero otherwise.  
\item \textbf{Bernoulli Sampling} -- Toss a weighted coin for each row, and take the row if the coin comes up heads (with probability $s$). 
\item \textbf{Uniform Sampling} -- Choose a number of rows $N_s = \lceil s \cdot N \rceil$.  Then, choose a subset of $N_s$ rows uniformly at random, without replacement. 
\item \textbf{Euclidean Sampling} -- Choose a number of rows $N_s = \lceil s \cdot N \rceil$.  Then, choose a subset of $N_s$ rows where the probability of choosing row $i$ is proportional to its Euclidean norm $\|K_i\|_2$ (again without replacement) \cite{frieze2004fast}.
\item \textbf{Distance Sampling} -- As in the Euclidean case, except the importance sampling distribution chooses row $i$ with probability inversely proportional to the distance of target point $i$ from the center of the sources. 
\item \textbf{Leverage Sampling} -- As in the Euclidean case, except that 
the probability of choosing a row is proportional to its leverage score (See Sec.~\ref{sec_theory}).
%\item \textbf{Mixture Sampling} -- Take a weighted combination of two (or more) other distributions, such as $90\%$ of the rows from a leverage score distribution and the remaining $10\%$ sampled uniformly. 
%\item \textbf{Tree-based sampling} -- Implement something like what I'm doing in the tree code.  Divide the points into some kind of tree data structure, then form the interaction list for the node containing my targets.  Sample a few points from each of these or something. 
\end{itemize}


\textbf{Kernels.} We show results on the following commonly used kernel functions:
\begin{itemize}
\item \textbf{Gaussian} -- characterized by a bandwidth $h$:
\begin{equation}
K_h(x, y) = \frac{1}{N h^d (2 \pi)^{\frac{d}{2}}} \exp \left( -\frac{1}{2 h^2} \|x - y\|^2 \right) 
\end{equation}
We can use an asymptotically optimal bandwidth from Silverman \cite{}:
\begin{equation}
h = something
\label{eqn_silverman_bandwidth}
\end{equation}
\item \textbf{Laplace}:
\begin{equation}
K(x,y) = \frac{1}{\|x - y\|}
\end{equation}
\item \textbf{Polynomial}:
\begin{equation}
K(x,y) = \left(\frac{x^T y}{\alpha} + c \right)^p
\end{equation}
\end{itemize}


%%%%%%%%%%%%%%%

\subsection{Kernels Can Be Compressed}

In order for our entire approach to be feasible, the subblocks of the full kernel matrix considered must be low-rank.  In Figure~\ref{fig_kernel_spectra}, we show the normalized singular values of $K$ for three different kernels for a range of dimensions. The Laplace kernel compresses particularly well, but all three show significant compression for the lower dimensions.  As the dimensionality grows, the Gaussian and polynomial kernels show less compression. 

\begin{figure}[tbph]
\centering
	\subfigure[Gaussian, $D_{\textrm{WS}} = 1$]{\includegraphics[width=0.3\textwidth]{figures/kernel_spectra/spectrum_gaussian_N_100000_m_100_WS_1.eps}}
	\subfigure[Laplace, $D_{\textrm{WS}} = 4$]{\includegraphics[width=0.3\textwidth]{figures/kernel_spectra/spectrum_laplace_N_100000_m_100_WS_4.eps}}
	\subfigure[Polynomial, $D_{\textrm{WS}} = 2$]{\includegraphics[width=0.3\textwidth]{figures/kernel_spectra/spectrum_polynomial_N_100000_m_100_WS_2.eps}}
\caption{The normalized singular values of the kernel matrix $K$ with $N = 10^5$ and $m = 100$.  The data are generated from a standard multivariate normal distribution.  The figures each display results for $d = 1, 2, 3, 4, 5, 8, 10$, which are in increasing order along the $y$ axis. The Gaussian kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}. The polynomial kernel uses $\alpha = 1.0, c = 0.1$, and $p = 3$.
\label{fig_kernel_spectra}}
\end{figure}


We then demonstrate that the SVD and ID can be used to successfully recover a typical kernel submatrix within the specified accuracy. In Figure~\ref{fig_basic_compression}, we show the relative error of our approximation (Eqn.~\ref{eqn_relative_approx_error}) for both the Gaussian and Laplace kernel. These experiments are simply compressing the full kernel matrix and do not involve any subsampling. 

In the three dimensional experiments, we see that the SVD outperforms the ID for both kernels, as expected. The difference in error between the methods is quite small, however, suggesting that the ID is an effective compression method. 
 The Gaussian kernel in five dimensions shows less favorable compression.  Note that the ID shows less error than the SVD because it is employing a higher-rank approximation. 
 So, these figures suggest that for our parameter settings, compressing the Gaussian kernel is more difficult than the Laplace kernel.  
 
 This seems counterintuitive, since the Gaussian quickly becomes insignificant as the distance between the points increases, while long range interactions are known to be significant in the Laplace case. 
 %We discuss this point further below. 

%Important claims: compression works, even in more than one dimension

% Figure 1: error vs. epsilon, no subsampling, SVD and ID
% Several dimensionalities
% RUNNING: basic_compression, basic_compression_laplace
\begin{figure}[tbph]
        \centering
        \subfigure[Gaussian kernel, $d = 3$. ]{\includegraphics[width=0.45\textwidth]{figures/basic_compression/basic_compression_gaussian_ws_1_m_500_d_3.eps}} 
        \subfigure[Laplace kernel, $d = 3$.]{\includegraphics[width=0.45\textwidth]{figures/basic_compression/basic_compression_laplace_ws_4_m_500_d_3.eps}} 
        \subfigure[Gaussian kernel, $d = 5$. ]{\includegraphics[width=0.45\textwidth]{figures/basic_compression/basic_compression_gaussian_ws_1_m_500_d_5.eps}} 
        \subfigure[Laplace kernel, $d = 5$.]{\includegraphics[width=0.45\textwidth]{figures/basic_compression/basic_compression_laplace_ws_4_m_500_d_5.eps}} 
\caption{Relative error vs. $\epsilon$ for different compression methods.  The data are generated from a standard multivariate normal distribution. Each experiment uses $N = 10^5$ and  $m = 500$. For the Gaussian, we use the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth} and $D_{\textrm{WS}} = 1$.  For the Laplacian, we use $D_{\textrm{WS}} = 4$.
\label{fig_basic_compression}}
\end{figure}



% Figure 2: Fixed epsilon, error vs. leaf size, 20 to 2000
% Several dimensionalities
% RUNNING: leaf_sizes, leaf_sizes_laplace

% leaf_sizes_gaussian ran out of memory -- figure out why and re-run
	% have them up to d = 5
	
We also examine increasing numbers of sources (values of $m$) in Figures~\ref{fig_leaf_sizes_gaussian} and \ref{fig_leaf_sizes_laplace}. If we are establishing the true rank of the kernel, then we should not see much change as $m$ increases. Once again, we observe that the Laplace kernel compresses extremely well, while the Gaussian does not. In both cases, the error from the ID is within a small constant factor of the optimal SVD error. 

\begin{figure}[tbph]
        \centering
        \subfigure[$d = 3$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_error_gaussian_ws_1_d_3_eps_-2.eps}} 
        \subfigure[$d = 3$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_rank_gaussian_ws_1_d_3_eps_-2.eps}} 
        \subfigure[$d = 5$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_error_gaussian_ws_1_d_5_eps_-2.eps}} 
        \subfigure[$d = 5$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_rank_gaussian_ws_1_d_5_eps_-2.eps}} 
        %\subfigure[$d = 10$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_error_gaussian_ws_1_d_10_eps_-2.eps}} 
        %\subfigure[$d = 10$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_rank_gaussian_ws_1_d_10_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $\epsilon = 10^{-2}$ and $D_{\textrm{WS}} = 1$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}. The first column displays the relative error and the second is the rank of the approximation used.
\label{fig_leaf_sizes_gaussian}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$d = 3$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_error_laplace_ws_4_d_3_eps_-2.eps}} 
        \subfigure[$d = 3$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_rank_laplace_ws_4_d_3_eps_-2.eps}} 
        \subfigure[$d = 5$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_error_laplace_ws_4_d_5_eps_-2.eps}} 
        \subfigure[$d = 5$.]{\includegraphics[width=0.45\textwidth]{figures/leaf_sizes/leaf_sizes_rank_laplace_ws_4_d_5_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $\epsilon = 10^{-2}$ and $D_{\textrm{WS}} = 1$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  The first column displays the relative error and the second is the rank of the approximation used.
\label{fig_leaf_sizes_laplace}}
\end{figure}


%%%%%%%%%%%%%%%%%%%

\subsection{Kernels Can Be Compressed Seeing Only a Few Rows}

Having established that kernel sub matrices can be accurately captured (in the 2-norm sense) from a low-rank interpolative decomposition, we now examine our results on sub-sampling  kernel matrices. 
The key claim here is that we can compute a low rank approximation by examining
only a small fraction of the rows of $K$. We show results for several values of $\epsilon$ and $d$ and for the polynomial, Laplace, and Gaussian kernels in Figures~\ref{basic_subsampling_gaussian_d_1} through \ref{basic_subsampling_polynomial_d_5_ws2}.

In lower dimensions, all kernels show excellent compression for $s = 10^{-3}$.  For a given error tolerance, we can find an interpolative decomposition from a small fraction of the rows that is nearly as accurate as one that sees the entire matrix. Unsurprisingly, the more sophisticated sampling methods based on importance distributions outperform the naive ones. 

In higher dimensions, the Gaussian subsampling again breaks down. However, even in these cases, we can determine the best possible approximation from a small fraction of the rows. 

There is a weird peak at $s = 10^{-1}$. It is not clear why this is happening. 



% Figure: The compression ones I've been showing 

% Also, ones showing the rank to be fixed --- RUNNING: fixed_rank_gaussian, fixed_rank_laplace
% forgot the different sampling methods for Gaussian, re-running them now


%Important claims: sampling works, importance sampling is necessary, distance is a good proxy for the better sampling scores

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_1_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_1_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_1_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 1$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{basic_subsampling_gaussian_d_1}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_2_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_2_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_2_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 2$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{basic_subsampling_gaussian_d_2}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_3_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_3_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_3_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 3$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{basic_subsampling_gaussian_d_3}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_5_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_5_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_5_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 5$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{basic_subsampling_gaussian_d_5}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_8_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_8_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_gaussian_ws_1_m_500_d_8_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 8$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{basic_subsampling_gaussian_d_8}}
\end{figure}

%%%%%%%

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_1_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_1_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_1_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 1$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_laplace_d_1}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_2_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_2_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_2_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 2$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_laplace_d_2}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_3_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_3_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_3_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 3$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_laplace_d_3}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_5_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_5_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_5_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 5$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_laplace_d_5}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_8_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_8_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_laplace_ws_4_m_500_d_8_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 8$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_laplace_d_8}}
\end{figure}


%%%%%%%%%%

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_1_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_1_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_1_eps_-2.eps}} 
\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 2$, $d = 1$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_polynomial_d_1_ws2}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_2_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_2_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_2_eps_-2.eps}} 
\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 2$, $d = 2$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_polynomial_d_2_ws2}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_3_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_3_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_3_eps_-2.eps}} 
\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 2$, $d = 3$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_polynomial_d_3_ws2}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_4_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_4_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_4_eps_-2.eps}} 
\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 2$, $d = 4$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_polynomial_d_4_ws2}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_5_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_5_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_2_m_500_d_5_eps_-2.eps}} 
\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 2$, $d = 5$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{basic_subsampling_polynomial_d_5_ws2}}
\end{figure}


%%%%%

%
%
%\begin{figure}[tbph]
%        \centering
%        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_1_eps_-8.eps}} 
%        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_1_eps_-4.eps}} 
%        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_1_eps_-2.eps}} 
%\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 4$, $d = 1$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
%\label{basic_subsampling_polynomial_d_1}}
%\end{figure}
%
%\begin{figure}[tbph]
%        \centering
%        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_2_eps_-8.eps}} 
%        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_2_eps_-4.eps}} 
%        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_2_eps_-2.eps}} 
%\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 4$, $d = 2$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
%\label{basic_subsampling_polynomial_d_2}}
%\end{figure}
%
%\begin{figure}[tbph]
%        \centering
%        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_3_eps_-8.eps}} 
%        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_3_eps_-4.eps}} 
%        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_3_eps_-2.eps}} 
%\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 4$, $d = 3$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
%\label{basic_subsampling_polynomial_d_3}}
%\end{figure}
%
%\begin{figure}[tbph]
%        \centering
%        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_4_eps_-8.eps}} 
%        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_4_eps_-4.eps}} 
%        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_4_eps_-2.eps}} 
%\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 4$, $d = 4$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
%\label{basic_subsampling_polynomial_d_4}}
%\end{figure}
%
%\begin{figure}[tbph]
%        \centering
%        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_5_eps_-8.eps}} 
%        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_5_eps_-4.eps}} 
%        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/basic_subsampling/basic_subsampling_id_polynomial_ws_4_m_500_d_5_eps_-2.eps}} 
%\caption{Polynomial kernel ($\alpha = 1.0, c = 0.1, p = 3$) compression experiments with $D_{\textrm{WS}} = 4$, $d = 5$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
%\label{basic_subsampling_polynomial_d_5}}
%\end{figure}
%
%



\textbf{Controlling for Rank.} These experiments (Figures~\ref{fixed_rank_gaussian_d_1} through \ref{fixed_rank_laplace_d_8}) choose the rank of the approximation via the number of singular values greater than $\epsilon \cdot \sigma_1(K_s)$, where $K_s$ is the subsampled matrix.  We also consider matrices where the normalization factor $\sigma_1(K)$ is known in advance.  In these experiments, the approximate rank is computed as the number of singular values of $K_s$ that are larger than $\epsilon \cdot \sigma_1(K)$, so that the cutoff no longer depends on the sample chosen.



\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_1_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_1_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_1_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 1$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{fixed_rank_gaussian_d_1}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_2_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_2_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_2_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 2$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{fixed_rank_gaussian_d_2}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_3_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_3_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_3_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 3$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{fixed_rank_gaussian_d_3}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_5_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_5_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_5_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 5$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{fixed_rank_gaussian_d_5}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_8_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_8_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_gaussian_ws_1_m_500_d_8_eps_-2.eps}} 
\caption{Gaussian kernel compression experiments with $D_{\textrm{WS}} = 1$, $d = 8$, and $m = 500$. The data are generated from the standard multivariate normal distribution. The kernel uses the bandwidth in Eqn.~\ref{eqn_silverman_bandwidth}.  
\label{fixed_rank_gaussian_d_8}}
\end{figure}

%%%%%%%

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_1_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_1_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_1_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 1$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{fixed_rank_laplace_d_1}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_2_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_2_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_2_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 2$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{fixed_rank_laplace_d_2}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_3_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_3_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_3_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 3$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{fixed_rank_laplace_d_3}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_5_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_5_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_5_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 5$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{fixed_rank_laplace_d_5}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-8}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_8_eps_-8.eps}} 
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_8_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.3\textwidth]{figures/fixed_rank/fixed_rank_id_laplace_ws_4_m_500_d_8_eps_-2.eps}} 
\caption{Laplace kernel compression experiments with $D_{\textrm{WS}} = 4$, $d = 8$, and $m = 500$. The data are generated from the standard multivariate normal distribution.  
\label{fixed_rank_laplace_d_8}}
\end{figure}



%%%%%%%%%%%%%%%%%%%



\subsection{We Can Handle Low-Dimensional Data Embedded in High-Dimensions}

One of the key motivations of our work is that existing methods do not scale well with increasing dimensionality of the data.  However, our results so far suggest that kernel matrices derived from high dimensional data do not compress effectively.  

In this section, we examine results on experiments in which the data are in a high ambient dimension, but are actually captured by a small number of dimensions. We generate points from a multivariate standard normal distribution in $d_i$ dimensions.  We then pad these data with zeros so that they are in $d_e$ dimensions, where $d_e > d_i$. We apply a random rotation, then add uniformly distributed noise. Results on this data set are presented in figures \ref{low_intrinsic_gaussian} and \ref{low_intrinsic_laplace}.

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.45\textwidth]{figures/low_intrinsic/low_intrinsic_id_gaussian_ws_1_m_100_d_100_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.45\textwidth]{figures/low_intrinsic/low_intrinsic_id_gaussian_ws_1_m_100_d_100_eps_-2.eps}} 
\caption{
Gaussian kernel compression where $d_i = 3, d_e = 100, m = 100$, and $D_{WS} = 1$.
\label{low_intrinsic_gaussian}}
\end{figure}

\begin{figure}[tbph]
        \centering
        \subfigure[$\epsilon  = 10^{-4}$.]{\includegraphics[width=0.45\textwidth]{figures/low_intrinsic/low_intrinsic_id_laplace_ws_4_m_100_d_100_eps_-4.eps}} 
        \subfigure[$\epsilon  = 10^{-2}$.]{\includegraphics[width=0.45\textwidth]{figures/low_intrinsic/low_intrinsic_id_laplace_ws_4_m_100_d_100_eps_-2.eps}} 
\caption{
Laplace kernel compression where $d_i = 3, d_e = 100, m = 100$, and $D_{WS} = 4$.
\label{low_intrinsic_laplace}}
\end{figure}

As these results demonstrate, our method can successfully compress these matrices, despite no prior information about the true dimensionality of the data.



%
%% Figure: compression of 4-d Gaussian in 10000 D or something
%
%
%
%
%%%%%%%%%%%%%%%%
%
%\subsection{Experiments in the Literature}
%
%\textbf{Improved FGT} -- \cite{yang2003improved}. -- All Gaussian kernels.
%
%Uniform unit cube sources and targets. Gaussian bandwidth $h = 0.2$. $\epsilon = 0.02$, $d = 3$. 
%
%Uniform unit cube sources and targets. $d = 4, 6, 8, 10; h = 1$, $N$ up to $10^4$. 
%Also, normal distribution, scaled into unit hypercube.
%



==> lafmm_sisc_outline.tex <==




New Story, 1/31

Kernel summation is important: KDE, SVM, computational physics

Solve them with tree codes / FMM
Pictures and brief description -- approximate the interactions between two distant groups of points
	Need an incoming and outgoing representation
We focus on the outgoing for simplicity

Analytic version of rep. -- original FMM
KIFMM / ID -- more general
	These are built with fictitious targets -- requires $O(m^{d-1})$ target points (and the ability to create new targets)
What if we directly compress the kernel submatrix?
	seems too expensive, rest of the paper is about doing this tractably 
	
	
	
Randomized linear algebra is a powerful tool for doing this.  The best results on approximating a matrix fall into two categories.
	Random projections -- too expensive, if we could do a matvec, we would already be done
	Direct sampling -- effective methods require an importance distribution, which is also too expensive
	
We look at sampling rows without an importance distribution in the context of forming outgoing representations for tree codes and the FMM

We show a theoretical argument from a different direction than existing sampling results.  We show that for low coherence matrices, naive sampling is as good as sampling from a carefully constructed importance distribution. This result is of independent interest as well.
We also show numerical results indicating that our approach is effective on real data sets. 


Questions:
How do we choose l? How do we know that we have enough samples without knowing the coherence?

	



























%^%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%^%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%^%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%^%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

INTRODUCTION

Kernel sums are important
	Lots of different kernels come up from physics, PDE's, ML
	New ones are being invented and learned in the ML literature all the time
	Some of them are over weird types, like strings or graphs

Really big ones are important too -- big data and simulations
	This is a problem because of quadratic scaling

Fast methods exist -- FMM, etc.
	But, these require detailed knowledge about the kernel

A recent method was proposed to overcome this restriction 
	Just do linear algebraic decompositions on the off-diagonal blocks of the kernel matrix 
		in principle, this requires no prior knowledge about the kernel beyond how to evaluate it and that off-diagonal blocks will have low rank
	This has only been demonstrated in one dimension and requires assumptions about interpolation of the kernel
	
We explore approaches to extend this methods to higher dimensions and fewer restrictions on the kernel
	In particular, we apply recent explorations in randomized methods for linear algebraic decompositions 
		These methods have been used recently to great success in obtaining approximate matrix-matrix products and low-rank decompositions of large matrices

We provide the first exploration of the application of these ideas to the task of accelerating matrix-vector products. 
	This requires special consideration, since existing randomized LA routines often read the entire matrix as a preprocessing step, while we cannot even form the entire matrix.

We provide the following contributions: etc.


%% Need to work more on making our problem seem important
	% drive home that its at the intersection of two very important things
	
	

LINEAR ALGEBRAIC FMM

-- Introduce the Interpolative Decomposition

Outline the method

Write up description of translation operators
Write up algorithm itself
Write something about the runtime of the algorithm -- key point: as written it's as slow as direct (or worse).  How do we speed this up?
	They use interpolation -- doesn't generalize. 
	We try randomization.


RANDOMIZED LINEAR ALGEBRA

Give the lit survey here
Stress that no one has worked on these cheaper matvecs, and they usually read the whole matrix





THEORY

Add citations for matrix coherence -- Mahoney? did he introduce it first?






EXPERIMENTS






DISCUSSION AND CONCLUSIONS



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Small to-do items:
Rework the definition of ID, cite something more thorough than Cheng et al.





==> lafmm_sisc_randomized_LA.tex <==


Randomized algorithms have recently emerged as a powerful tool in numerical linear algebra. 
We focus on a subset of these algorithms for computing approximate, compact (or otherwise computationally efficient) representations of a matrix.
Throughout, we approximate a matrix $A \in \reals^{m \times n}$.  We seek to approximate $A$ with some matrix $\hat{A}$, typically of rank exactly or approximately $k$.

The gold standard for such representations is the truncated singular value decomposition.  It is well-known that the matrix $A_k = U_k \Sigma_k V_k^T$ consisting of the first $k$ singular vectors and values of $A$ provides the following approximation errors:
\begin{eqnarray}
\|A - A_k\|_F & = & \sum_{i = k+1}^n \sigma_i \\
\|A - A_k\|_2 & = & \sigma_{k+1}
\end{eqnarray}
and that these errors are the best possible for any rank $k$ approximation. 
However, the truncated SVD typically requires $O(m n k)$ work in most cases \cite{gu1996efficient}.

Another decomposition of interest is the interpolative decomposition (ID), discussed previously. Rather than computing a new basis for the approximate subspace, the ID chooses columns or rows of the input matrix to serve as such a basis. Such a decomposition can be obtained through a rank revealing QR factorization and satisfies the following bound:
\begin{equation}
\|A - A_{\textrm{col}} P \|_2 \leq \sqrt{1 + l k(l - k)} \sigma_{k+1}(A)
\end{equation}
with $l = \min\{m , n\}$.
This factorization also typically requires $O(m n k)$ work \cite{cheng2005compression}. 
The ID is also related to the column subset selection problem, in which the task is to choose the $k$ columns of $A$ which best approximate $A$ in the Frobenius or spectral norm sense. 

Randomized algorithms seek to compute approximate representations more efficiently, while preserving the favorable error guarantees of the direct methods. 
These methods can be generally divided into two categories: random projection methods and subsampling methods.  Throughout, we focus on the case of interest to us: namely one in which the number of rows is much larger than the number of columns.  All of the results discussed can be generalized from this case in a straightforward way. 

Randomized algorithms have also been successfully applied to many other tasks in linear algebra, including least-squares solutions of overdetermined systems \cite{}, non-negative matrix factorizations \cite{}, matrix-matrix multiplication \cite{}, $\ell_p$ regression \cite{}, 

\subsection{Random projections} 
%Random projections are a powerful tool for efficient randomized algorithms.  Essentially, these methods work by projecting a high-dimensional object into a lower dimensional space while preserving properties of interest.  
The Johnson-Lindenstrauss lemma states that points in $N$ dimensional Euclidean space can be embedded in $O(\log N)$ dimensions while approximately preserving the Euclidean distances between the points \cite{johnson1984extensions}.  Furthermore, it holds that a projection onto a set of $O(\log N)$ iid random Gaussian vectors satisfies this property with high probability \cite{dasgupta2003elementary}. 
The application of this idea to the efficient computation of matrix decompositions is straightforward.  We first project the matrix $A$ into some smaller $l$-dimensional space, then compute a decomposition of the projected matrix.  This approach was first taken by Sarlos \cite{sarlos2006improved}, who showed that this method can compute a $(1 + \epsilon)$ relative error approximation in the Frobenius norm. 
Extensions of this method use structured random projections which can be applied more efficiently while preserving favorable error guarantees \cite{sarlos2006improved, ailon2006approximate, tropp2008conditioning, tropp2008norms, tropp2011improved}.  These methods have been specifically applied in the context of efficient matrix approximation \cite{martinsson2011randomized, woolfe2008fast}.

While random projections have excellent error guarantees, they require us to project the original matrix onto the span of some random vectors.  Even for structured random projections, this will generally require us to at least touch all of the entries of the matrix.  Since our ultimate goal is to provide a sub-quadratic algorithm for matrix-vector multiplication, this is prohibitively expensive.


%%%%%%%%%

These bounds are from the survey paper of Halko et al \cite{halko2011finding}.
\begin{theorem}
Choose a rank $k$ and oversampling parameter $p$. Draw a standard Gaussian matrix $\Omega \in \reals^{n \times (k + p)}$ and let $Y = A \Omega$. Then,
\begin{equation}
\mathbb{E} \|(I - P_Y) A\|_F \leq \left( 1 + \frac{k}{p-1} \right)^{\frac{1}{2}} \left( \sum_{j > k} \sigma_j^2 \right)^\frac{1}{2}
\end{equation}
\begin{equation}
\mathbb{E} \|(I - P_Y) A\|_2 \leq \left( 1 + \sqrt{\frac{k}{p-1}} \right) \sigma_{k+1} + \frac{e \sqrt{k+p}}{p} \left( \sum_{j > k} \sigma_j^2 \right)^\frac{1}{2}
\end{equation}
\end{theorem}

They also provide tail bound versions of these bounds. 
\begin{theorem}
Under the same hypotheses, along with $p \geq 4$.  Then, for all $u, t \geq 1$, 
\begin{equation}
\|(I - P_Y) A\| \leq \left[ \left( 1 + t \cdot \sqrt{12k/p} \right) \sigma_{k+1} + t \cdot \frac{e \sqrt{k + p}}{p + 1} \left( \sum_{j > k} \sigma_j^2 \right)^\frac{1}{2} \right] + ut \cdot \frac{e \sqrt{k+p}}{p+1} \sigma_{k+1}
\end{equation}
with probability at most $5 t^{-p} + e^{-u^2/2}$. 
\end{theorem}
Note that my bounds are an improvement over any of these. No one has given column selection bounds in this kind of context. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Subsampling from the matrix}
The other major thread in randomized linear algebra concerns the direct subsampling of entries of the matrix. 
One of the earliest methods approximates the matrix by sampling individual entries \cite{achlioptas2001fast, achlioptas2007fast}. 
%\begin{theorem}
%\cite{achlioptas2001fast}.  Let $A \in \reals^{m \times n}$ and $b = \max_{i,j} |A_{i,j}|$.  For $1 \leq s \leq (m + n) / (4 \log^6(m + n))$, let $\hat{A}$ be defined by $\hat{A}_{i,j} = s A_{i,j}$ with probability $1/s$ and 0 otherwise.  Then, with probability at least $1 - 1 / (m+n)$,
%\begin{equation}
%\|A - \hat{A}_k \| < \|A - A_k\| + \sqrt{s} \times 10 b \sqrt{m + n}
%\end{equation}
%where $A_k$ denotes the best rank $k$ approximation to $A$ obtained from the SVD.
%\label{thm_achlioptas_entrywise_sampling}
%\end{theorem}
%This approach has been applied in the context of kernel PCA \cite{scholkopf2002sampling} and optimization \cite{d2008subsampling} as well.
While the resulting sparsity of the subsampled matrix may be desirable for some applications, we require a method that preserves the relationships between entries in a row or column, since these represent the potential due to a source or at a target

%\begin{table}
%\centering
%\caption{Results on constructing a low-rank approximation from a subset of rows or columns. Let $\mathcal{E}$ be the approximation error of the optimal rank $k$ matrix in the norm being considered.
%\label{table_randomized_la_results}}
%\begin{tabular}{} \hline
%Reference & Norm (2 or F) & Bound & Number of samples \\
%
%Frieze, \emph{et al.} \cite{frieze2004fast} & $F$ & $\mathcal{E} + \frac{10 k}{s} \sum_{i=1}^N \sigma_i^2$ & $s$ \\
%
%Rudelson \cite{rudelson2007sampling} & 
%
%Deshpande. \emph{et al.} \cite{deshpande2006adaptive} & $F$ & $(1 + \epsilon) \mathcal{E}$ \\
%
%\hline
%\end{tabular}
%\end{table}
%

Another line of work, originating with Frieze, Kannan and Vempala \cite{frieze2004fast}, samples entire rows or columns of the original matrix. By drawing a subset of the columns or rows from some carefully chosen distribution, these methods preserve the action of the matrix while reducing its dimensionality to something manageable. 
Algorithms in this line of work produce bounds of the form
\begin{theorem}
\cite{frieze2004fast}. Let $A$ be $m \times n$ and let $S$ be a set of $s$ rows of $A$ sampled independently from a distribution such that the probability $P_i$ of sampling row $i$ satisfies
\begin{equation}
P_i \geq \frac{|A^{(i)}|^2}{\|A\|^2_F}
\end{equation}
for all $i$.
Let $V$ be the spaced spanned by the vectors in $S$. Then with probability at least $0.9$, there exist a set of orthonormal vectors $y_1, \ldots, y_k \in V$ such that 
\begin{equation}
\left\| A - A \left(\sum_{j=1}^k y_j y_j^T \right) \right\|_F^2 \leq \min_{D, \textrm{rank}(D) \leq k} \|A - D\|^2_F + \frac{10 k}{s} \|A \|_F^2
\end{equation}
\label{thm_fkv_row_sampling}
\end{theorem}


A similar result was proved for the 2-norm by Rudelson and Vershynin \cite{rudelson2007sampling}. 
\begin{theorem}
\cite{rudelson2007sampling}. Let $A$ be $m \times n$ such that is has rank $r = \|A\|_F^2 / \|A\|_2^2$. Let $d \leq m$ be such that 
\begin{equation}
d \geq C \left( \frac{r}{\epsilon^4 \delta} \right) \log \left(\frac{r}{\epsilon^4 \delta} \right)
\end{equation}
Choose $d$ rows of $A$ with probability proportional to their Euclidean lengths and scale them appropriately. Then, for any integer $k$, with probability at least $1 - 2 \exp(-c / \delta)$, we have that
\begin{equation}
\|A - A P_k\|_2 \leq \sigma_{k+1}(A) + \epsilon \|A\|_2
\end{equation}
\end{theorem}
They claim that this is an improvement in sample complexity over \cite{drineas2006fast2}. 


Further work along these lines utilizes more sophisticated sampling distributions. 
The intuition behind the above approach is that rows with larger 2-norm will have a greater on the range and spectrum of the matrix.  However, if a new sample lies in the span of the previous samples, it doesn't tell us anything new about the range of the matrix. Therefore, we can sample more efficiently if we update the sampling probabilities such that the $j^{\textrm{th}}$ sample is chosen with probability
\begin{equation}
p_i^{(j)} = \frac{\|E^{(i)}_j\|^2}{\|E_j\|^2_F} 
\label{eqn_adaptive_sampling}
\end{equation}
where $E_j = A - \pi_{\cup S_k}$ is the part of $A$ not accounted for by the previous samples.  
This approach is first presented in \cite{deshpande2006matrix} and extended in \cite{deshpande2006adaptive}.  Using this adaptive sampling, they show that the additive error of Thm.~\ref{thm_fkv_row_sampling} can be reduced exponentially.  
\begin{theorem}
\textbf{\cite{deshpande2006adaptive}.}  Any $m \times n$ matrix $A$ contains a subset $S$ of $4k / \epsilon + 2 k \log (k + 1)$ rows such that there is a matrix $\hat{A}_k$ of rank $k$ in the span of $S$ such that
\begin{equation}
\|A - \hat{A}_k\|^2_F \leq (1 + \epsilon) \|A - A_k\|_F^2
\end{equation}   
\end{theorem}
This would seem to be the tightest possible bound.  

Another productive body of work, used in the results in this paper, utilizes the concept of statistical leverage scores to form an importance sampling distribution \cite{drineas2006subspace, drineas2006subspace2, drineas2006polynomial, drineas2006fast, drineas2006fast2, drineas2006fast3, boutsidis2009improved, drineas2004clustering, mahoney2012randomized}.  These methods have also appeared in the machine learning literature as ``Nystrom methods'' \cite{drineas2005nystrom, talwalkar2010matrix}.
Importance sampling distributions based on the magnitudes of rows of the matrix of right or left singular vectors can provide the best existing methods for matrix subsampling approximations.  Existing results in this area are all of the form: given $O(k \log k)$ samples from a distribution where the probability of a row is proportional to its leverage score, we can obtain a tight approximation.  


















==> sampling.tex <==
\textbf{Sampling extras.}
Uniform sampling based on the tree data structure was applied in the
context of an algorithm for kernel
summations \cite{kapur1998ies3,kapur1997fast}.  

This approach was
further explored by computing the discretization of the SVD of the
(infinite dimensional) kernel operator
itself \cite{yarvin1998generalized, yarvin1999improved,
gimbutas2003generalized}; there the sampling is not random but
corresponds to quadrature points.  This approach is successful in low
dimensions, but fails in higher dimensions for reasons discussed
in~\S\ref{subsec_interpolation}.



==> svd_interpolation_crap.tex <==
Given an SVD of the kernel function on appropriate subdomains or an ID
%
\rmrg{
This section is unconnected to the rest. Trim down everything up to the last equation of the SVD.}
of kernel matrix subblocks, we can implement the outgoing representation for a treecode. 

 We now turn to the key step in this method, the construction of these
decompositions.  We begin with the SVD in one
dimension. Following \cite{yarvin1999improved}, we can build the SVD
using a combination of interpolation and quadrature.

We focus on the construction of an outgoing representation of a set of
sources $S$, contained in an interval $[a, b]$.
%
\lmrg{Why 1D? Use
 $[\delta/2,1]^d$ and  $[-\delta/2,-1]^d$.}
%GB in this way we can connect the errors to $\delta$ and the previous
%section. 

% Don't use d here -- that's the dimension
 Let $[c, d]$ be the
region for which we want the outgoing representation to hold. In
general, we will want this representation to hold to the left and
right of the source interval.
\rmrg{If you change the dimension, fix notation}
 We will build a representation for one side, and we can then repeat
the process for the other.  Combining these two representations yields
the final outgoing representation. 
\rmrg{This may be incorrect. G. thinks it only uses one SVD.}

Let $\Ker$ be a square integrable
kernel function.
\lmrg{This is introduced suddenly.}

We require a quadrature and interpolation scheme for each interval
which satisfy the following conditions: the nodes of the quadrature
and interpolation schemes are identical, the interpolation scheme is
linear, and the quadrature can exactly compute the integral of the
product of any two outputs of the interpolation.
\rmrg{The point is not clear here.}
%
Let the nodes of the
schemes on $[a, b]$ be $x_1, \ldots, x_n$, the weights of the
quadrature be $w_1, \ldots, w_n$, and the interpolation functions be
$\alpha_1, \ldots, \alpha_n$. Similarly, let the nodes for $[c, d]$ be
$y_1, \ldots, y_m$, the weights $v_1, \ldots, v_m$, and the functions
$\beta_1, \ldots, b_m$.
%
\rmrg{Notation: $v_k$ used for weights and singular functions}
%
Given these, we can generalize the SVD of the matrix of interactions
between interpolation points to an SVD of the kernel operator.  We
first compute the $n \times m$ matrix
\begin{equation}
K_{ij} = \Ker(x_i, y_j) \sqrt{w_i v_j}
\end{equation}

We then compute the rank $p$ truncated SVD of $K \approx U_p \Sigma_p
V^T_p$, and scale the singular vectors by
\begin{eqnarray}
\hat{u}_{ik} & = & U_{ik} / \sqrt{w_i} \\
\hat{v}_{jk} & = & V_{jk} / \sqrt{v_j}
\end{eqnarray}
We then define functions $u_k$ and $v_k$ by:
\begin{eqnarray}
u_k(x) & = & \sum_{i = 1}^n \hat{u}_{ik} \alpha_i(x) \\
v_k(y) & = & \sum_{j = 1}^m \hat{v}_{jk} \beta_j(y)
\end{eqnarray}
\lmrg{Notation: $n$ and $m$ are used in the text. Use something different here.}

Then, the SVD of the operator $\Ker$ on the intervals $[a, b]$ and $[c, d]$ can be approximated as 
\begin{equation}
\tilde{\Ker}(x, y) \approx \sum_{k = 1}^p \sigma_k u_k(x) v_k(y)
\end{equation}
and the error is related to interpolation and quadrature.  In other
words, this function is exactly equal to computing the kernel function
directly from the two interpolation schemes:
\begin{equation}
\tilde{\Ker}(x, y) = \sum_{i = 1}^n \sum_{j = 1}^m K(x_i, y_j) \alpha_i(x) \beta_j(y).
\end{equation}
\lmrg{What is the point of this equation? }

